MoORE: SVD-based Model MoE-ization for Conflict- and Oblivion-Resistant Multi-Task Adaptation

Adapting large-scale foundation models in multi-task scenarios often suffers from task conflict and oblivion. To mitigate such issues, we propose a novel ''model MoE-ization'' strategy that leads to a conflict- and oblivion-resistant multi-task adaptation method. Given a weight matrix of a pre-trained model, our method applies SVD to it and introduces a learnable router to adjust its singular values based on tasks and samples. Accordingly, the weight matrix becomes a Mixture of Orthogonal Rank-one Experts (MoORE), in which each expert corresponds to the outer product of a left singular vector and the corresponding right one. We can improve the model capacity by imposing a learnable orthogonal transform on the right singular vectors. Unlike low-rank adaptation (LoRA) and its MoE-driven variants, MoORE guarantees the experts' orthogonality and maintains the column space of the original weight matrix. These two properties make the adapted model resistant to the conflicts among the new tasks and the oblivion of its original tasks, respectively. Experiments on various datasets demonstrate that MoORE outperforms existing multi-task adaptation methods consistently, showing its superiority in terms of conflict- and oblivion-resistance. The code of the experiments is available at https://github.com/DaShenZi721/MoORE.

==> supp_arxiv.tex <==

\appendix

\section{Hyperparameters and Implementation Details}\label{app:set}

The detailed hyperparameter setups are presented in Table~\ref{tab:appset}. 
Both training and testing are conducted on one NVIDIA A100 GPU.

\begin{table}[htbp]
  \centering
  \caption{Hyperparameter configurations of MoORA on the CSR-MTL and the NLU-MTL.}
    \begin{tabular}{l|c}
    \toprule
    Hyperparameters & MoORA \\
    \midrule
    Cutoff Length & 512 \\
    Batch Size & 8\;/\;64 \\
    Epochs & 2\;/\;5 \\
    Learning Rate & 3E-04 \\
    LR scheduler & Warmup-Stable-Decay \\
    Warmup Ratio & 5\% \\
    Decay Ratio & 5\% \\
    Optimizer & AdamW \\
    Dropout Rate & 0.0  \\
    \midrule
    Target Modules & Q, K, V, O, Up, Down, Gate \\
    $D_{t}$ & 128 \\
    $D_{s}$ & 64 \\
    $L$ & 8 \\
    \bottomrule
    \end{tabular}%
  \label{tab:appset}%
\end{table}%
\section{Tasks and Datasets}\label{app:data}

Detailed information about the CSR-MTL, the NLU-MTL and the OR-MTL is presented in Tables~\ref{tab:appcs}, Table~\ref{tab:appglue} and Table~\ref{tab:appor}, respectively.
These tables include the sizes of the training and test sets, as well as the task types.

\begin{table}[htbp]
  \centering
  \caption{The basic information of CSR-MTL.}
    \begin{tabular}{l|ccc}
    \toprule
    Task Name & \#Train & \#Test & Task Type \\
    \midrule
    ARC-Challenge & 1,119 & 1,172 & Question Answering \\
    ARC-Easy & 2,250 & 2,380 & Question Answering \\
    BoolQ & 9,427 & 3,270 & Text Classification \\
    OpenBookQA & 4,957 & 500 & Question Answering \\
    PIQA & 16,100 & 1,840 & Question Answering \\
    SocialIQA & 33,410 & 1,954 & Question Answering \\
    HellaSwag & 39,905 & 10,042 & Sentence Completion \\
    WinoGrande & 9,248 & 1,267 & Fill in the Blank \\
    CommonsenseQA & 9,741 & 1,140 & Question Answering \\
    \bottomrule
    \end{tabular}%
  \label{tab:appcs}%
\end{table}%

\begin{table}[htbp]
  \centering
  \caption{The basic information of NLU-MTL.}
    \begin{tabular}{l|ccc}
    \toprule
    Task Name & \#Train & \#Validation & Task Type \\
    \midrule
    CoLA & 8,551 & 1,043 & Text Classification \\ 
    MNLI & 392,702 & 9,815 & - \\
    MRPC & 3,668 & 408 & - \\
    QNLI & 104,743 & 5,463 & - \\
    QQP & 363,846 & 40,430 & - \\
    RTE & 67,350 & 873 & - \\
    SST-2 & 2,491 & 277 & - \\
    \bottomrule
    \end{tabular}%
  \label{tab:appglue}%
\end{table}%

\begin{table}[htbp]
  \centering
  \caption{The basic information of OR-MTL.}
    \begin{tabular}{l|cc}
    \toprule
    Task Name & \#Test & Task Type \\
    \midrule
    MMLU & 14,042 & Question Answering \\ 
    IFEval & 541 & Text Generation \\
    BBH & 6,511 & Question Answering \\ 
    GPQA & 448 & Question Answering \\ 
    HumanEval & 164 & Text Generation \\ 
    MBPP & 500 & Text Generation \\ 
    GSM-8K & 1,319 & Text Generation \\ 
    \bottomrule
    \end{tabular}%
  \label{tab:appor}%
\end{table}%

\section{More Experimental Results}

\subsection{Performance on other Model Architectures in Conflict-Resistance}\label{app:qwen}

To evaluate the cross-model performance of MoORE, we take Qwen-2.5 7B as the backbone model and apply various MoE-based multi-task adaptation methods to it. 
Experimental results on CSR-MTL are shown in Table~\ref{tab:qwen}.
We can find that MoORE outperforms baselines consistently under different hyperparameter settings, and the performance of MoORE is robust to the change of $L$. 
These results verify the robustness of our method and its compatibility with various model architectures.


\begin{table}[htbp]
  \centering
  \caption{Results (\%) of Qwen-2.5 7B adapted by various methods on CSR-MTL. The best results on each dataset are shown in \textbf{bold}, and the second best results are shown in \underline{underline}.}
  \tabcolsep=2pt
  \small{
    \begin{tabular}{l|c|ccccccccc|c}
    \toprule
    Method & \#Params & ARC-C & ARC-E & BoolQ & OBQA & PIQA & SIQA & HellaS & WinoG & CSQA & Overall \\
    \midrule
    LoRA~\cite{hu2021lora} & 2.12\% & 87.29 & 91.88 & 70.37 & 90.60 & 87.92 & 79.02 & 92.73 & 74.98 & 84.36 & 84.35 \\
    MixLoRA~\cite{li2024mixlora} & 3.32\% & 86.86 & 91.75 & 71.38 & 91.40 & 89.28 & 80.45 & 95.06 & 78.45 & 85.09 & 85.53 \\
    MoSLD~\cite{zhao2025mosld} & 1.43\% & 86.69 & 92.13 & 71.96 & 90.40 & 89.66 & 80.40 & 95.17 & 78.30 & \textbf{85.50} & 85.58 \\
    HydraLoRA~\cite{tian2024hydralora} & 2.83\% &  \underline{88.23} & 91.54 & 72.57 & 91.20 & 85.80 & 80.09 & \underline{95.95} & \textbf{82.24} & \underline{85.26} & 85.87 \\
    MTL-LoRA~\cite{yang2025mtl} & 2.80\% & 87.80 & 92.09 & 72.72 & \underline{92.20} & 86.07 & 79.79 & 95.92 & 80.66 & 84.36 & 85.73 \\
    LoRAMoE~\cite{dou2024loramoe} & 2.21\% & 87.20 & 91.84 & \textbf{73.61} & 90.40 & \textbf{90.37} & \textbf{81.27} & \textbf{95.99} & 80.27 & 84.60 & 86.17 \\
    \midrule
    MoORE$_{\; L=0}$ & 2.29\% & 88.06 & 92.17 & \underline{73.49} & \underline{92.20} & \textbf{90.37} & 79.58 & 95.40 & \underline{81.53} & 84.03 & 86.31 \\
    MoORE$_{\; L=2}$ & 2.32\% &  \underline{88.23} & \underline{92.34} & 73.09 & 91.60 & \underline{90.32} & 80.60 & 95.50 & 81.45 & 84.19 & 86.37 \\
    MoORE$_{\; L=4}$ & 2.35\% & \textbf{88.40} & 92.21 & 73.18 & 91.40 & 90.21 & \textbf{81.27} & 95.25 & 80.58 & 84.93 & \underline{86.38} \\
    MoORE$_{\; L=16}$ & 2.53\% &  \underline{88.23} & \textbf{92.59} & 73.30 & \textbf{92.40} & 90.26 & \underline{81.12} & 95.50 & 81.37 & 84.93 & \textbf{86.63} \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:qwen}%
\end{table}%

\subsection{Numerical Performance in Oblivion-Resistance}\label{app:oblivion}

Following LLaMA-3.1 8B, we select MMLU~\cite{hendryckstest2021,hendrycks2021ethics}, IFEval~\cite{zhou2023instructionfollowingevaluationlargelanguage}, BIG-Bench Hard~(BBH)~\cite{suzgun2022challenging}, GPQA~\cite{rein2024gpqa}, HumanEval~\cite{chen2021evaluating}, MBPP~\cite{austin2021program}, and GSM-8K~\cite{cobbe2021gsm8k} as evaluation tasks and adopt the same few-shot settings.
More detailed results of the oblivion-resistance experiments are presented in Table~\ref{tab:appforget}, corresponding to the results shown in Figures~\ref{fig:increment2} and~\ref{fig:forget}. 


\begin{table}[htbp]
  \centering
  \caption{The loss of performance in the original tasks. Each method is represented by two rows of data: the first row indicates the performance on the current task, while the second row shows the difference between the post-fine-tuning score and the pre-fine-tuning score.}
  \tabcolsep=3pt
  \small{
    \begin{tabular}{l|c|c|c|c|c|c|c|c}
    \toprule
    Category & \multicolumn{3}{c|}{General} & \multicolumn{1}{c|}{Reasoning} & \multicolumn{2}{c|}{Code} & Math & \\
    \midrule
    Task & MMLU & IFEval & BBH & GPQA & HumanEval & MBPP & GSM-8K & Overall \\
    \midrule
    % Metric &  macro\_avg/acc & & & exact\_match & \multicolumn{2}{c|}{pass@1} & em\_maj1@1 & \\
    % \midrule
    \#Shots &  5 &  & 0 & 0 & 0 & 3 & 8 & \\
    \midrule
    Llama-3.1-8B-Instruct & 68.15 & 84.53 & 46.09 & 34.15 & 56.71 & 59.00 & 85.52 & 62.02 \\
    \midrule
    \multirow{2}{*}{LoRA} & 32.40 & 29.14 & 13.65 & 27.23 & 0.00 & 0.00 & 2.12 & 14.93 \\ 
    & -35.75 & -55.39 & -32.44 & -6.92 & -56.71 & -59.00 & -83.40 & -47.09 \\
    \midrule
    \multirow{2}{*}{LoRAMoE} & 63.74 & 78.06 & 34.16 & 31.47 & 60.98 & 57.40 & 78.54 & 57.76 \\
    & -4.41 & -6.47 & -11.93 & -2.68 & 4.27 & -1.60 & -6.98 & -4.26\\
    \midrule
    \multirow{2}{*}{MoSLD} & 61.77 & 75.06 & 34.74 & 28.57 & 56.10 & 53.60 & 70.05 & 54.27 \\
    & -6.38 & -9.47 & -11.35 & -5.58 & -0.61 & -5.40 & -15.47 & -7.75 \\
    \midrule
    \multirow{2}{*}{MTL-LoRA} & 61.55 & 72.30 & 31.59 & 31.92 & 57.32 & 51.60 & 66.57 & 53.26  \\
    & -6.60 & -12.23 & -14.50 & -2.23 & 0.61 & -7.40 & -18.95 & -8.76 \\
    \midrule
    \multirow{2}{*}{HydraLoRA} & 62.34 & 69.78 & 30.27 & 30.36 & 54.27 & 54.80 & 66.41 & 52.60 \\
    & -5.81 & -14.75 & -15.82 & -3.79 & -2.44 & -4.20 & -19.11 & -9.42 \\
    \midrule
    \multirow{2}{*}{MixLoRA} & 64.47 & 77.82 & 38.21 & 30.13 & 54.27 & 56.20 & 74.83 & 56.56 \\
    & -3.68 & -6.71 & -7.88 & -4.02 & -2.44 & -2.80 & -10.69 & -5.46 \\
    \midrule
    \multirow{2}{*}{MoORE} & 65.32 & 82.49 & 40.21 & 31.92 & 66.46 & 58.20 & 80.36 & 60.71 \\
    & -2.83 & -2.04 & -5.88 & -2.23 & 9.75 & -0.80 & -5.16 & -1.31 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:appforget}%
\end{table}%



\subsection{Ablation Study}\label{app:ablation}
To analyze the impact of the task-level routing, sample-level routing, and orthogonal adapter quantitatively, we conduct ablation study on the CSR-MTL dataset. 
In Table~\ref{tab:ablation}, we record the overall performance achieved when only one of these three modules is applied.
In particular, without the orthogonal adapter, our method degrades to the MoE with fixed experts.
When merely applying the orthogonal adapter without any routing, our method is simplified as the single-task adaptation method HRA~\cite{yuan2024bridging}.
The results show that when only one of these three modules is applied, even with a wider network and more trainable parameters, the model's performance declines significantly across the entire dataset.
These results demonstrate that all these three modules contribute to the overall effectiveness of MoORE.

\begin{table}[t]
  \centering
  \caption{Ablation studies of MoORE on CSR-MTL. \faTimes \; indicates the absence of that component.}
  \tabcolsep=5pt
  \small{
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
    Method & $D_{t}$ & $D_{s}$ & $L$ & \#Params & Overall \\
    \midrule
     & 16 & \faTimes & \faTimes & 0.14\% & 79.55 \\
    Merely Apply & 32 & \faTimes & \faTimes & 0.29\% & 81.80 \\
    Task-level Routing& 64 & \faTimes & \faTimes & 0.58\% & 83.06 \\
     & 128 & \faTimes & \faTimes & 1.16\% & 83.53 \\
    \midrule
     & \faTimes & 16 & \faTimes & 0.39\% & 82.30 \\
    Merely Apply & \faTimes & 32 & \faTimes & 0.78\% & 82.91 \\
    Sample-level Routing& \faTimes & 64 & \faTimes & 1.57\% & 83.57\\
     & \faTimes & 128 & \faTimes & 3.13\% & 83.80 \\
    \midrule
    & \faTimes & \faTimes & 2 & 0.03\% & 80.76 \\
    Merely Apply & \faTimes & \faTimes & 4 & 0.06\% & 82.15 \\
    Orthogonal Adapter& \faTimes & \faTimes & 8 & 0.12\% & 82.98 \\
     & \faTimes & \faTimes & 16 & 0.25\% & 83.90 \\
    \midrule
    MoORE & 128 & 64 & 8 & 2.84\% & 85.11 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:ablation}%
\end{table}%
% \begin{wrapfigure}{r}{0.4\textwidth}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/speed.pdf}
%     \caption{The comparison for various methods on inference efficiency.}
%     \label{fig:speed}
% \end{wrapfigure}

% To evaluate the inference efficiency of different methods, we measure their inference speed on the GPQA task within the Language Model Evaluation Harness
% framework. 
% The inference speed is calculated by dividing the total inference time by the number of inference samples. 
% For fairness, the adapters of each method are merged into the original weight matrices (except for the adapter experts in MoE, which cannot be merged). 
% Specifically, for MoORE, we integrate the orthogonal adapter into each expert.  
% The results shown in Figure~\ref{fig:speed} indicate that MoORE achieves inference efficiency comparable to the best-performing method MixLoRA.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/routing_weights_stem_hellaswag.pdf}
    \caption{The mean and variance of routing weights obtained in HellaS.}
    \label{fig:approuter1}
\end{figure}

\subsection{Analysis of Routing Weights}\label{app:weight}

To investigate the router's preferences for the experts in MoORE, we analyze the distribution of routing weights across different tasks in the CSR-MTL dataset.
Take the $Q$ module from the first attention layer of the adapted model as an example.
For each task, we compute and show the mean (red point) and variance (blue stem) of each expert's weight over all samples of the task in Figures~\ref{fig:approuter1} and~\ref{fig:approuter3}.
In each figure, the mean weight of an expert is shown as a red point, and the blue stem associated with the point shows the standard deviation.
These visualization results provide us with some insights in the mechanism behind MoORE:
\begin{itemize}[left=5pt]
    \item \textbf{Preference on the originally important experts.} 
    Compared to other components, the routing weights corresponding to the principal components of $\bm{W}$ (i.e., the experts corresponding to large singular values) are adjusted more significantly.
    The routing weights corresponding to the significant experts are distributed relatively symmetrically around the zero scale, whereas the routing weights for the minor components are more concentrated above the zero scale. 
    This indicates that the model tends to focus on adjusting the routing weights of the experts that are important in the pre-training phase.
    In other words, these originally important experts often maintained their significance when adapting for new task.
    % \item
    % This suggests that during multi-task adaptation, the model both discards and enhances well-learned pre-training knowledge.
    % In contrast, for the less-optimized subspace spanned by the minor singular vectors, the model primarily focuses on learning.
    % This indicates that the model acquires knowledge that was either not learned or weakly learned during pretraining.
    \item Based on the mean and variance of the routing weights, the nine tasks in CSR-MTL can be grouped into three categories:  
    \begin{itemize}
        \item \textbf{Large Mean, Large Variance:} Tasks such as Hellaswag fall into this group. 
        MoORE performs well on the Hellaswag.
        A large mean indicates that the model significantly enhances or discards well-learned pretraining knowledge, while a large variance means that the model can capture substantial differences between samples and assign different experts to them with high flexibility.  
        \item \textbf{Small Mean, Large Variance:} Tasks such as OBQA, PIQA, SIQA, and CSQA belong to this group.
        This result indicates that for each of these tasks, its samples have significant diversity, and MoORE needs to activate different experts to handle different samples.
        \item \textbf{Small Mean and Variance:} Tasks such as ARC-C, ARC-E, BoolQ, and Winogrande (WinoG) are in this group. 
        Except for ARC-E, MoORE performs poorly on these tasks.
        A small mean indicates minimal adjustment to pretraining knowledge, and a small variance suggests minor differences between samples. 
        For the relatively simple ARC-E task, the model may have already mastered the ability to solve it, requiring little adjustment.
        However, for the more challenging tasks in this group, the model may struggle to learn the ability to solve them within the column space spanned by the singular vectors.
    \end{itemize}
\end{itemize}

\begin{figure}[t]
    \centering
    \subfigure[OBQA]{
    \includegraphics[width=0.95\linewidth]{figures/routing_weights_stem_obqa.pdf}
    }
    \subfigure[PIQA]{
    \includegraphics[width=0.95\linewidth]{figures/routing_weights_stem_piqa.pdf}
    }
    \subfigure[SIQA]{
    \includegraphics[width=0.95\linewidth]{figures/routing_weights_stem_siqa.pdf}
    }
    \subfigure[CSQA]{
    \includegraphics[width=0.95\linewidth]{figures/routing_weights_stem_csqa.pdf}
    }
    \caption{The mean and variance of routing weights obtained in four QA tasks.}
    \label{fig:approuter2}
\end{figure}
\begin{figure}[t]
    \centering
    \subfigure[ARC-C]{
    \includegraphics[width=0.95\linewidth]{figures/routing_weights_stem_arc-c.pdf}
    }
    \subfigure[ARC-E]{
    \includegraphics[width=0.95\linewidth]{figures/routing_weights_stem_arc-e.pdf}
    }
    \subfigure[BoolQ]{
    \includegraphics[width=0.95\linewidth]{figures/routing_weights_stem_boolq.pdf}
    }
    \subfigure[WinoG]{
    \includegraphics[width=0.95\linewidth]{figures/routing_weights_stem_winogrande.pdf}
    }
    \caption{The mean and variance of routing weights obtained in the remaining four tasks of CSR-MTL.}
    \label{fig:approuter3}
\end{figure}

\section{Broader Impacts}\label{sec:appimpact}
MoORE can effectively enhance the performance of LLMs in multi-task adaptation and facilitate the application of LLMs in real-world scenarios.
Similar to other multi-task adaptation methods, such as MixLoRA and HydraLoRA, MoORE may result in some potential negative social impacts, such as the risk of abuse for adapting LLMs in illegal activities. 
However, these issues are not unique to MoORE --- other adaptation methods are also susceptible to similar risks.
Addressing these issues thoroughly will require advancements in technology, the establishment of relevant legal frameworks, and shifts in societal perspectives.
